Towards an Integrated Performance Framework for Fire Science and Management Workflows

Reliable performance metrics are necessary prerequisites to building large-scale end-to-end integrated workflows for collaborative scientific research, particularly within context of use-inspired decision making platforms with many concurrent users and when computing real-time and urgent results using large data. This work is a building block for the National Data Platform, which leverages multiple use-cases including the WIFIRE Data and Model Commons for wildfire behavior modeling and the EarthScope Consortium for collaborative geophysical research. This paper presents an artificial intelligence and machine learning (AI/ML) approach to performance assessment and optimization of scientific workflows. An associated early AI/ML framework spanning performance data collection, prediction and optimization is applied to wildfire science applications within the WIFIRE BurnPro3D (BP3D) platform for proactive fire management and mitigation.

==> graveyard.tex <==
% DO NOT DELETE
Contributions of the paper:

- a performance framework for integrating data and machine learning on top of open CI to improve scalability and reliability (responsible AI, reproducibility, reuseability, trustworthiness)

- An implemented architecture to collect and analyze performance data as an AI-ready service

- Examples toward predictive modeling techniques for performance provision of AI workflows





% DO NOT DELETE --- AI-readiness approach outline (by Ravi)
\textbf{Prerequisites}
    \begin{enumerate}
        \item  For each run, make sure input parameters, run-ids, and ensemble-ids are stored somewhere you can access
        \item In Kubernetes or wherever runs are being hosted/run, their names include an ensemble-id or run-id (preferred) in a consistent manner.
        \item Performance metrics are stored in some database such that there is an ability to query performance metrics at any point in time for past runs. This is where Nautilus and PromQL comes in.
    \end{enumerate}

\textbf{Collecting Data}
      \begin{enumerate}
          \item Get a list of all runs and their inputs to use as training data.
          \item Drop all failed runs (NA values in run start, run end, or sim time), saving them to a new spreadsheet for later models on guessing which pods will be dropped
          \item Decide on metrics to collect, then use PromQL to query for those metrics using nautilus API
          \begin{enumerate}
              \item Get metrics by Node, Pod in query to be able to get run ids from pod names and information about which nodes are trustworthy.
          \end{enumerate}
          \item Get queries working for a specified time range using duration and offset in PromQL
          \item Once Queries can query over a particular time range, use them to get data for every bp3d run in training data set. Add a column to the training data for each queried metric. Put the newly collected data into its respective column. It will be in a JSON-like format.
          \begin{enumerate}
              \item Choose the metrics that you want to be able to predict. Query these metrics over the entire run. These columns will act as an 'answer key' of sorts for your model. 
          \end{enumerate}
          \item Decide on user-interaction with the model. Two main options:
          \begin{enumerate}
              \item Model refreshes predictions at set times
              \item User can refresh predictions starting at a certain time (once there is current performance data to base predictions from) and then any time onward.
          \end{enumerate}
    \end{enumerate}

\textbf{Implementation of user-interaction choice}
Model refreshes predictions at set times:
\begin{itemize}
    \item For each metric, query over the time range from the start time until each set time. Add each one as a column.
    \item As an example, let's say if I have predictions refresh at 1 minute, 5 minutes, 15 minutes, and 1 hour. Focusing on just CPU usage to simplify things, I will create 4 columns as well as the run's total CPU usage. These four columns will be cpu-t1, cpu-t2, cpu-t3 and cpu-t4. The model will take in these columns and guess CPU total.
\end{itemize}

User can refresh predictions:
\begin{itemize}
    \item Add a new column for a user refresh time. Then add a column cpu-t1 querying from start time until that refresh time. 
    \item You can add as many refresh columns and corresponding metric columns per run as you would like, but keep in mind you don't want your model to over fit the data. 
    \begin{itemize}
        \item Then when training the model, only pass one refresh column and its corresponding metric columns at a time.
    \end{itemize}
    \item For creating the refresh columns, keep in mind when users are most likely to refresh the predictions and generate refresh times randomly more often during those likely refresh times. 
    \begin{itemize}
        \item For example, Our first refresh column is between 45 seconds (when refresh option will first be available) and 300 seconds (5 minutes). There is a strong likelihood that users will want a more accurate prediction within the first 5 minutes of the run.
    \end{itemize}
\end{itemize}

\textbf{Getting Data to a Usable Format}
\begin{enumerate}
    \item For every run in training data, get run id from path where bp3d run was stored.
    \item For each queried performance column, sum over all the pods for the current run to get a single float instead of a list of dictionaries. In an ideal scenario, run-ids are encoded into the pod name.
\begin{itemize}
    \item In that case, take the run-id for the run, and for every pod in  the list of dictionaries, if that pod contains the run-id, add it to the total. Replace the JSON-like entry with the total float value.
\end{itemize}

    \begin{itemize}
        \item Note: our Kubernetes pods were not named in this ideal fashion. Ours have ensemble-ids encoded, so we have to sum over all pods with the ensemble id but only during the time of the run.
        \begin{itemize}
            \item This has no difference if  the simulation ran sequentially, but if there are multiple threads running at the same time, some of the resource usage from other runs will be included in what is collected for this run. 
            \item Thus, in our case, there may be a correlation between number of threads and over-reporting metric data.
        \end{itemize}
    \end{itemize}
    
    \item Calculate certain values from input columns to make it easier for a model.
    \begin{itemize}
        \item For example, given four simulation corner points, calculate the area. Add area as a new column, drop the corner points column.
    \end{itemize}
    
    \item Select all useful columns for the training data. Drop all the others. Use data exploration and knowledge of the simulation to know which data columns are useful and which are unnecessary.
    \begin{itemize}
        \item Once you have all of the useful data collected in an ML-friendly format, you are ready to start choosing and training a model.
    \end{itemize}
\end{enumerate}





%Sample table and figure: 

\begin{table}[htbp]
\caption{Table Type Styles}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Table}&\multicolumn{3}{|c|}{\textbf{Table Column Head}} \\
\cline{2-4} 
\textbf{Head} & \textbf{\textit{Table column subhead}}& \textbf{\textit{Subhead}}& \textbf{\textit{Subhead}} \\
\hline
copy& More table copy$^{\mathrm{a}}$& &  \\
\hline
\multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\begin{figure}[htbp]
\centerline{\includegraphics{fig1.png}}
\caption{Example of a figure caption.}
\label{fig}
\end{figure}


